Accurate and Efficient Trajectory-based Contact Tracing with Secure Computation and Geo-Indistinguishability

Contact tracing has been considered as an effective measure to limit the transmission of infectious disease such as COVID-19. Trajectory-based contact tracing compares the trajectories of users with the patients, and allows the tracing of both direct contacts and indirect contacts. Although trajectory data is widely considered as sensitive and personal data, there is limited research on how to securely compare trajectories of users and patients to conduct contact tracing with excellent accuracy, high efficiency, and strong privacy guarantee. Traditional Secure Multiparty Computation (MPC) techniques suffer from prohibitive running time, which prevents their adoption in large cities with millions of users. In this work, we propose a technical framework called ContactGuard to achieve accurate, efficient, and privacy-preserving trajectory-based contact tracing. It improves the efficiency of the MPC-based baseline by selecting only a small subset of locations of users to compare against the locations of the patients, with the assist of Geo-Indistinguishability, a differential privacy notion for Location-based services (LBS) systems. Extensive experiments demonstrate that ContactGuard runs up to 2.6$\times$ faster than the MPC baseline, with no sacrifice in terms of the accuracy of contact tracing.

==> sections/background.tex <==
\section{Background} 
\label{sec:background}

We introduce the background on the Secure Multiparty Computation (MPC) and the Geo-indistinguishability in this section. 

\subsection{Secure Multiparty Computation (MPC)}
\label{subsec:smc}

Secure Multiparty Computation (MPC) allow multiple parties to jointly compute the desired function outputs over their private inputs, without revealing each party's private inputs to any other parties. The strong privacy guarantee it offered is that only the function output is released, and no other information is disclosed. Thus, the input data by each party is strictly protected. 

It achieves the protection of the input data by encryption. The output is derived from the encrypted input data collectively over all parties. Any single party could not derive the final output, and the single party could not access the plaintext of other parties because of the encryption. 

In addition, the computation process (the process of evaluating the function output) is \textit{oblivious} \cite{he2021practical}. The instruction traces, program counters and the execution time are independent of the private inputs. This ensures that at any step during the computation, nothing about the private inputs are disclosed. 

The standard steps for achieving MPC starts by representing the computation of the desired function outputs as a circuit. There are two common ways to represent the computation as oblivious circuit \cite{zahur2015obliv}. One way is through a data-oblivious Boolean logic circuit, which includes logic gates (\eg AND, OR). The logic gates are specified without knowing the private inputs.  The second way is to use addition and multiplication gates (as opposed to the AND, OR gates) which operate on finite field elements. 

After representing the computation as a circuit, a secure protocol is used to encrypt the private data to be used in the evaluation in the circuit. The protocol ensures that the circuit is executed without revealing any private inputs or the intermediate results. Finally, the secure protocol is executed by evaluating the gates within the circuit, following the topological orders of the designed circuit \cite{he2021practical}. 


\subsection{Geo-indistinguishability}
\label{subsec:geo-i}

Geo-indistinguishability (Geo-I) \cite{andres13} extends the traditional and well-adopted privacy notion -- differential privacy \cite{DBLP:conf/icalp/Dwork06} to location-based systems. 

\begin{definition} (Geo-I) \label{def:geo-i} For all true locations $x,x'$, a privacy parameter $\epsilon$, a mechanism $M$ satisfies  $\epsilon$-Geo-I iff:
\begin{equation}
	d_{\rho}(M(x),M(x'))\leq \epsilon d(x,x'), \label{eq:geo_i_def}
\end{equation}
\end{definition}
where $d(x,x')$ is the Euclidean distance between $x$ and $x'$ while $d_{\rho}(M(x),M(x'))$ is the multiplicative distance between two distributions $M(x)$ and $M(x')$. $M(x)$ and $M(x')$ are the distributions of perturbed locations based on the original location $x$ and $x'$ respectively.

One particular mechanism satisfying Geo-I is drawing random noise from the planar Laplace distribution \cite{andres13} . Given the privacy parameter $\epsilon \in \mathbb{R}^{+}$, the actual location $x_0 \in \mathbb{R}^{2}$, the probability density function of a noisy location $x \in \mathbb{R}^{2}$ is:

\begin{equation}
D_\epsilon(x_0)(x)=\frac{\epsilon ^2}{2\pi}e^{-\epsilon d(x_0,x)} \\, \label{eq:geo_i_equation}
\end{equation}

where $\frac{\epsilon ^2}{2\pi}$ is the normalization factor. Examples of the planer Laplace distribution are given in \figref{fig:laplace}. 


\begin{figure}[t]
	\centering \vspace{0ex}
	   \begin{subfigure}[b]{0.49\textwidth}
		   \centering
		   \includegraphics[width=\textwidth]{figures/laplace_eps_0_2.pdf}
		   \caption{$\epsilon=0.2, l=(0,0)$.}
		   \label{subfig:laplace}
	   \end{subfigure}
	   \hfill
		\begin{subfigure}[b]{0.49\textwidth}
		   \centering
		   \includegraphics[width=\textwidth]{figures/laplace_eps_0_5.pdf}
		   \caption{$\epsilon=0.5, l=(1,1)$.}
		   \label{subfig:laplace_2}
	   \end{subfigure}
	\figureCaptionMargin
	\caption{\small The pdf of the planar Laplace distribution.}	
	\figureBelowMargin\vspace{0ex}
	\label{fig:laplace}
   \end{figure}




